Lectures on the Bondi--Metzner--Sachs group and related topics in infrared physics

These are the extended lecture notes for a minicourse presented at the I S\~ao Paulo School on Gravitational Physics discussing the Bondi--Metzner--Sachs (BMS) group, the group of symmetries at null infinity on asymptotically flat spacetimes. The BMS group has found many applications in classical gravity, quantum field theory in flat and curved spacetimes, and quantum gravity. These notes build the BMS group from its most basic prerequisites (such as group theory, symmetries in differential geometry, and asymptotic flatness) up to modern developments. These include its connections to the Weinberg soft graviton theorem, the memory effect, its use to construct Hadamard states in quantum field theory in curved spacetimes, and other ideas. Advanced sections briefly discuss the main concepts behind the infrared triangle in electrodynamics, superrotations, and the Dappiaggi--Moretti--Pinamonti group in expanding universes with cosmological horizons. New contributions by the author concerning asymptotic (conformal) Killing horizons are discussed at the end.

==> abbrvs.tex <==
\newabbreviation[shortplural={ACKHs},longplural={asymptotic conformal Killing horizons}]{ACKH}{ACKH}{asymptotic conformal Killing horizon}
\newabbreviation[shortplural={A(C)KHs},longplural={asymptotic (conformal) Killing horizons}]{A(C)KH}{A(C)KH}{asymptotic (conformal) Killing horizon}
\newabbreviation{AdS}{AdS}{anti-de Sitter}
\newabbreviation[shortplural={AKHs},longplural={asymptotic Killing horizons}]{AKH}{AKH}{asymptotic Killing horizon}
\newabbreviation{AQFT}{AQFT}{algebraic quantum field theory}
\newabbreviation{BHT}{BHT}{black hole thermodynamics}
\newabbreviation{BMS}{BMS}{Bondi--Metzner--Sachs}
\newabbreviation{CCR}{CCR}{canonical commutation relations}
\newabbreviation[shortplural={CFTs},longplural={conformal field theories}]{CFT}{CFT}{conformal field theory}
\newabbreviation{CK}{CK}{Christodoulou--Klainerman}
\newabbreviation{CMB}{CMB}{cosmical microwave background}
\newabbreviation{DC}{DC}{direct current}
\newabbreviation{DMP}{DMP}{Dappiaggi--Moretti--Pinamonti}
\newabbreviation{FLRW}{FLRW}{Friedmann--Lemaître--Robertson--Walker}
\newabbreviation{GR}{GR}{general relativity}
\newabbreviation[shortplural={GUTs},longplural={grand unified theories}]{GUT}{GUT}{grand unified theory}
\newabbreviation[shortplural={GWs},longplural={gravitational waves}]{GW}{GW}{gravitational wave}
\newabbreviation{HEP}{HEP}{high-energy physics}
\newabbreviation{IR}{IR}{infrared}
\newabbreviation{KAGRA}{KAGRA}{Kamioka Gravitational Wave Detector}
\newabbreviation{LHC}{LHC}{large hadron collider}
\newabbreviation{LHS}{LHS}{left-hand side}
\newabbreviation{LIGO}{LIGO}{Laser Interferometer Gravitational-Wave Observatory}
\newabbreviation{LISA}{LISA}{Laser Interferometer Space Antenna}
\newabbreviation[shortplural={NGBs},longplural={Nambu--Goldstone bosons}]{NGB}{NGB}{Nambu--Goldstone boson}
\newabbreviation[shortplural={OPEs},longplural={operator product expansions}]{OPE}{OPE}{operator product expansion}
\newabbreviation{PSZ}{PSZ}{Pasterski--Strominger--Zhiboedov}
\newabbreviation[shortplural={QFTs},longplural={quantum field theories}]{QFT}{QFT}{quantum field theory}
\newabbreviation{QFTCS}{QFTCS}{quantum field theory in curved spacetime}
\newabbreviation{QM}{QM}{quantum mechanics}
\newabbreviation{RG}{RG}{renormalization group}
\newabbreviation{RHS}{RHS}{right-hand side}
\newabbreviation[shortplural={SCTs},longplural={special conformal transformations}]{SCT}{SCT}{special conformal tranformation}
\newabbreviation{SEC}{SEC}{strong energy condition}
\newabbreviation{SM}{SM}{standard model of particle physics}
\newabbreviation{SSB}{SSB}{spontaneous symmetry breaking}
\newabbreviation{TT}{TT}{transverse-traceless}
\newabbreviation{UV}{UV}{ultraviolet}
